Stereo Matching by Self-supervision of Multiscopic Vision

Self-supervised learning for depth estimation possesses several advantages over supervised learning. The benefits of no need for ground-truth depth, online fine-tuning, and better generalization with unlimited data attract researchers to seek self-supervised solutions. In this work, we propose a new self-supervised framework for stereo matching utilizing multiple images captured at aligned camera positions. A cross photometric loss, an uncertainty-aware mutual-supervision loss, and a new smoothness loss are introduced to optimize the network in learning disparity maps end-to-end without ground-truth depth information. To train this framework, we build a new multiscopic dataset consisting of synthetic images rendered by 3D engines and real images captured by real cameras. After being trained with only the synthetic images, our network can perform well in unseen outdoor scenes. Our experiment shows that our model obtains better disparity maps than previous unsupervised methods on the KITTI dataset and is comparable to supervised methods when generalized to unseen data. Our source code and dataset are available at https://sites.google.com/view/multiscopic.

==> includes/conclusion.tex <==
% !TEX root =  ../main.tex


% \vspace{-0.2cm}
\section{Conclusion}

In this paper, we exploit the image shape of multiscopic images to learn an end-to-end network to estimate the disparity map without ground-truth depth information. 
In a multiscopic structure, the images are captured with parallel, co-planar, and same-parallax camera angles, such that the pixel disparities are the same between the center image and any surrounding image. Self-supervision is obtained by taking advantage of this constrain.
The cross photometric loss, uncertainty-aware mutual-supervision loss, and smoothness loss are introduced to guide self-supervised learning. 
% Since there is no ground truth to fit, the network has to learn the true pattern and geometry shape of this task rather than overfitting the training data. 
As there is no public large multiscopic dataset, we build a new dataset composed of synthetic images rendered by 3D engines and real-world images captured by the multiscopic systems designed by ourselves. 
After being trained with only these indoor synthetic images, our network can obtain better disparity maps in the unseen outdoor KITTI dataset, compared to previous unsupervised methods. Additionally, our network is comparable to supervised approaches when evaluated on images different from the training set.

==> includes/dataset.tex <==
% !TEX root =  ../main.tex


\section{Multiscopic Dataset}

In this section, we introduce the details of our multiscopic vision system and describe how we build our multiscopic dataset in virtual environments and the real world.

In a multiscopic vision structure, multiple images are captured at axis-aligned camera positions, such that these images are taken with parallel optical axes on the same image plane, and with the same parallaxes, as shown in Fig.~\ref{fig:camera}. Multiscopic vision structure brings clear benefits to depth estimation. The disparity of a pixel from the center view to any surrounding view should be the same, which is a strong constraint to optimize the result. Additionally, the occluded regions in one view can be perceived from other views, in which case there are no occlusion problems for the entire multiscopic system \cite{wei2005asymmetrical, drouin2005geo}.

Some interesting research can be conducted in this setup. For instance, multiscopic images can be utilized for better image enhancement since there are more constraints to be enforced, such as super-resolution with multiple images \cite{li2010multi}. % or improving the brightness of images taken in the dark \cite{chen2018learning}.
Also, view synthesis \cite{zhou2018stereo} can be done in a multiscopic structure, such as predicting the right view provided with only the left and center views.

Since there is no available large dataset for multiscopic vision, we build a new dataset composed of 1200 scenes of synthetic multiscopic data rendered by 3D engines and 100 scenes of real images taken with real-world cameras.



\subsection{Synthetic Data}

The synthetic images are rendered using the 3D render engine Habitat-sim \cite{savva2019habitat} and SceneNet RGB-D \cite{McCormac:etal:ICCV2017}, with 3D models from Matterport3D \cite{Matterport3D}, Gibson \cite{xiazamirhe2018gibsonenv}, and ShapeNet \cite{chang2015shapenet}. Habitat-sim is used to render Matterport3D as well as Gibson, and SceneNet RGB-D is used to render ShapeNet. The models from Matterport3D and Gibson are collected from real indoor spaces by reconstruction from data acquired using real-world RGB cameras, depth cameras, and 3D scanning sensors. Most models within them are ordinary houses with daily-life objects like furniture, decorations, and instruments. The models from ShapeNet are some virtual indoor space models, in which we can randomly place all kinds of 3D object models, like toys, plants, cars, or even airplanes. So when we render the scenes using models from ShapeNet, we adjust the lighting condition randomly while we keep the light the same as the real world when we render the models from Matterport3D and Gibson.

There are more than 20K raw scenes of images. We remove the similar scenes and keep 1200 scenes in total that are unlike each other. This makes these 1200 scenes representative of visual variation.
% , from which we pick up various 1200 scenes in total that are unlike to each other, and remove the similar scenes.
For each scene in our dataset, there are five images taken with multiscopic vision structure, the center, left, right, bottom, and top view, as shown in Fig.~\ref{fig:dataset}. More scenes can be seen in the supplementary materials. The resolution of all images is $1280\times1080$, and every color image has its corresponding ground-truth disparity map. As a multiscopic structure, the baselines between the four surrounding images and the center image are the same and vary from 0.05 to 0.2 meters. The value range of the disparity maps is from 0 to 255.



\subsection{Real-world Data}

Real-world multiscopic data are taken with one or multiple RGB cameras. Multiscopic images require aligned camera locations, which is not easy to control. Therefore, to capture images in this structure, we design two architecture: 
The first architecture is composed of three identical cameras with Sony IMX322 inside, whose resolution is $1920\times1080$. These three cameras are aligned on a horizontal line, as displayed in Fig.~\ref{fig:realcam}(a). They are parallel, co-planar, and with the same baseline of 4 centimeters.
The second design is a moving-eye system. Although we utilize the same cameras, a multi-eye structure still suffers from the problem that the cameras' parameters are not exactly the same. To overcome this, we place one camera on a precision linear sliding rail and slide it horizontally on its image plane, as displayed in Fig.~\ref{fig:realcam}(b). In this system, three images are taken at three locations to obtain multiscopic images. The baselines of adjacent locations vary from 3 to 4 centimeters.

Images obtained by a moving-eye system have strictly identical parameters, but sliding a camera needs some time so that it cannot take images of dynamic scenes. Thus, we combine these two systems to build a real-world image dataset. There are 100 scenes of real-world images in our dataset. For every scene, there are the left, center, and right images, as shown in Fig.~\ref{fig:dataset}(c). More scenes are shown in the supplementary materials. Some images are cropped to reduce the vignette influence and remove messy environments, after which the resolutions vary from $1400\times1000$ to $1920\times1080$. For the real data, there is no ground-truth depth information.


==> includes/experiments.tex <==
% !TEX root =  ../main.tex


\setlength{\tabcolsep}{5pt}
\begin{table}[]
\centering
\begin{tabular}{c c c c}
\toprule
Method & \tabincell{c}{\#Infer \\ input} & \tabincell{c}{Train set\\D1-all}  & \tabincell{c}{Test set\\D1-all}  \\
\midrule
Zhou et al. 2017~\cite{zhou2017unsupervised} & $2$ & $9.91\%$ & $-$ \\
Godard et al. 2017~\cite{godard2017unsupervised} & $2$ & $9.194\%$ & $-$ \\
Li et al. 2018~\cite{li2018occlusion} & $2$ & $-$ & $8.98\%$ \\
Guo et al. 2018~\cite{guo2018learning} & $2$ & $7.06\%$ & $-$ \\
UnOS 2019~\cite{wang2019unos} & $2$ & $7.073\%$ & $-$ \\
UnOS 2019~\cite{wang2019unos} & $4$ & $5.943\%$ & $6.67\%$ \\
Wang et al. 2020~\cite{wang2020parallax} & $2$ & $-$ & $7.23\%$ \\
% Loop-Net 2020~\cite{kim2020loop} & $4$ & $6.72\%$ & $-$ \\
Flow2Stereo 2020~\cite{liu2020flow2stereo} & $2$ & $6.13\%$ & $6.61\%$ \\
Ours & $2$ & $\mathbf{3.82\%}$ & $\mathbf{4.43\%}$  \\
\midrule
PSMNet & $2$ & $1.83\%$ & $2.32\%$  \\
PSMNet* & $2$ & $5.90\%$ & $-$  \\
\bottomrule
\end{tabular}%
\caption{Quantitative evaluation on the KITTI 2015 dataset. D1-all is the percentage of stereo disparity outliers in all regions of the first frame. End-point error smaller than $3$ pixels or $5\%$ is considered correct.}
\label{tab:kitti}
\vspace{-0.5cm}
\end{table}
\setlength{\tabcolsep}{3pt}


% \setlength{\tabcolsep}{5pt}
% \begin{table*}[]
% \centering
% \begin{tabular}{c c c c c c}
% \toprule
% Method & \tabincell{c}{Gound \\ truth} & \tabincell{c}{\#Input \\ images} & \tabincell{c}{Tuned on \\ KITTI} & \tabincell{c}{Train set\\D1-all}  & \tabincell{c}{Test set\\D1-all}  \\
% \midrule
% Zhou et al. 2017~\cite{zhou2017unsupervised} & \xmark & $2$ & Yes & $9.91\%$ & $-$ \\
% Godard et al. 2017~\cite{godard2017unsupervised} & \xmark & $2$ & Yes & $9.194\%$ & $-$ \\
% Godard et al. 2017~\cite{godard2017unsupervised} & \xmark & $2$ & No & $11.36\%$ & $-$ \\
% Wang et al. 2019~\cite{wang2019unos} & \xmark & $2$ & Yes & $7.073\%$ & $-$ \\
% Wang et al. 2019~\cite{wang2019unos} & \xmark & $4$ & Yes & $5.943\%$ & $-$ \\
% Liu et al. 2020~\cite{liu2020flow2stereo} & \xmark & $2$ & Yes & $6.13\%$ & $6.61\%$ \\
% Ours & \xmark & $2$ & No & $\mathbf{4.32\%}$ & $\mathbf{5.00\%}$  \\
% \midrule
% % MC-CNN~\cite{zbontar2016stereo} & \cmark & $2$ & Yes & $3.25\%$ & $3.89\%$  \\
% % MC-CNN~\cite{zbontar2016stereo} & \cmark & $2$ & No & $4.49\%$ & $-$  \\
% PSMNet~\cite{chang2018pyramid} & \cmark & $2$ & Yes & $1.83\%$ & $2.32\%$  \\
% PSMNet~\cite{chang2018pyramid} & \cmark & $2$ & No & $5.90\%$ & $-$ \\
% \bottomrule
% \end{tabular}%
% \caption{Quantitative evaluation on the KITTI 2015 dataset. D1-all is the percentage of stereo disparity outliers in all regions of the first frame. End-point error smaller than $3$ pixels or $5\%$ is considered correct. ``Not tuned on KITTI" means trained on our synthetic data.}
% \label{tab:kitti}
% \vspace{-0.5cm}
% \end{table*}
% \setlength{\tabcolsep}{3pt}



\section{Experiments}

In this section, we first present the details of our experimental setup. Afterward, we evaluate our model on the synthetic test set, KITTI 2015 dataset, and real-world images. Also, ablation studies are performed to provide insight into the effect of each module in our framework.

\subsection{Implementation Details}

The self-supervised learning framework is implemented in Pytorch and trained on two Nvidia GTX 1080 Ti GPUs. The batch size is set to 4 and the weights $\lambda_1, \lambda_2, \lambda_3, \lambda_4$ are set to $1,0.01,0.03,0.03$. 
% Input images are normalized to have zero mean and one standard deviation before being fed into the network. 
Images are randomly cropped to $512\times256$ for every epoch during training to reduce the size and work as data augmentation. The network is optimized end-to-end with Adam ($\beta_1=0.9$, $\beta_1=0.999$) and the learning rate is set to $0.0001$.


Our network is only trained using 1,000 scenes of synthetic data. The performance trained with additional real multiscopic images is similar since our synthetic images are quite photo-realistic.
During training, three multiscopic images are used as the input of our learning framework because the performance of using five images is similar, and our real-world system captures three images. For evaluation, we only use two stereo images for depth estimation. Examples of the output $D_c^r$ between the right view and the center view of test images are shown in Fig.~\ref{fig:res-synthe}. The output disparity maps are very close to the ground truth disparity maps.



\subsection{Evaluation}

\subsubsection{Synthetic data} We build a synthetic test set consisting of 200 scenes of multiscopic images. After the training, we evaluate our model on these images to examine its performance on synthetic images. The center view and the right view are used as the input to the network. Four metrics are applied, and the results are summarized in Table~\ref{tab:synthetic}. The EPE is the average endpoint error, Bad$0.5$, Bad$1$, and Bad$2$ is the percentage of pixels whose error is higher than $0.5$, $1$, and $2$, respectively.

We also compare our method with some unsupervised and supervised methods when trained on our synthetic dataset, as presented in Table~\ref{tab:synthetic}. The results show that our method is better than the previous unsupervised method \cite{godard2017unsupervised} and comparable to the supervised method PSMNet. Qualitative results are displayed in Fig.~\ref{fig:res-synthe}.
Then, we test the performance of the original supervised models of the MC-CNN and PSMNet trained on the KITTI dataset. The errors of their outputs are high, which illustrates that the generalization ability of these supervised methods is not satisfactory.




\subsubsection{KITTI 2015}

To compare our method with other unsupervised or self-supervised approaches, we evaluate the trained model on the KITTI 2015 dataset \cite{geiger2012we}, which includes 200 training stereo images pairs and 200 test pairs. The ground truth for the test set is withheld for evaluation. From the quantitative results shown in Table~\ref{tab:kitti}, our method outperforms all previous unsupervised learning methods by a large margin even without fine-tuning on the KITTI data. In other words, our model is not trained on outdoor images but can perform well on outdoor images in the KITTI dataset. We believe our model could achieve a lower error if trained on KITTI-style multiscopic images. The D1-all error of Godard~\cite{godard2017unsupervised} trained with our synthetic images is $11.36\%$ while its error reduces to $9.194\%$ after the fine-tuning on KITTI images.
Also, the second-best performing method \cite{wang2019unos} utilizes two consecutive stereo pairs while we only use one pair.

Some qualitative results are displayed in Fig.~\ref{fig:res-kitti} for visualization. The results demonstrate the generalization ability of our method, which benefits from self-supervised learning. In self-supervised learning, since there is no ground truth depth information, there is no chance to overfit the depth value. Instead, the network needs to find the inner pattern and geometry shape underneath.

% We also compare our results with the supervised method MC-CNN (accurate model). As reported in their paper, when they train the network with KITTI 2015 data, the D1 error on KITTI 2015 validation set is $3.25\%$. However, the error is $4.49\%$ when trained on Middlebury data and $3.99\%$ when trained on KITTI 2012 data. This means if not trained on the same dataset, the performance of this supervised method does not have advantages over our unsupervised approach. Even the data in KITTI 2012 is very similar to KITTI 2015, generalization from KITTI 2012 to KITTI 2015 still suffers from a large performance decrease. This shows the drawback of supervised learning methods. Still, state-of-the-art supervised method PSMNet can reach much lower error when it is trained on the same dataset since it can fit the data.

We also compare our results with the supervised method PSMNet when trained on our synthetic dataset without fine-tuning on the KITTI images, denoted as ``PSMNet*". When the model is trained with KITTI data, the D1 error on KITTI 2015 can reach $1.83\%$. However, the error is $5.90\%$ when trained on our synthetic training set. This means if not trained on the same dataset, the performance of this supervised method does not have advantages over our self-supervised approach. Generalization between different datasets suffers from a large performance decrease, which is the drawback of supervised learning methods.


\begin{figure}[t]
\centering
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/slider16aview1}
\end{subfigure}
%
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/slider16dispcolor}
\end{subfigure}
%
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/slider16dispcolor-psm}
\end{subfigure}

\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/slider18aview1}
  \caption*{Color image}
\end{subfigure}
%
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/slider18dispcolor}
  \caption*{Our model}
\end{subfigure}
%
\begin{subfigure}{0.32\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/slider18dispcolor-psm}
  \caption*{PSMNet}
\end{subfigure}
%
% \begin{subfigure}{0.45\columnwidth}
%   \centering
%   \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/slider17aview1}
% \end{subfigure}
% %
% \begin{subfigure}{0.45\columnwidth}
%   \centering
%   \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/slider17dispcolor}
% \end{subfigure}
%
% \begin{subfigure}{0.45\columnwidth}
%   \centering
%   \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/slider28aview1}
%   \caption*{Center view}
% \end{subfigure}
% %
% \begin{subfigure}{0.45\columnwidth}
%   \centering
%   \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/slider28dispcolor}
%   \caption*{Output $D_c^r$}
% \end{subfigure}
% \vspace{-0.3cm}
\caption{Test on real images in our dataset. The output of our model and the supervised method PSMNet are presented.}
\label{fig:res-real}
\vspace{-0.5cm}
\end{figure}


\subsubsection{Real-world Data and Online Fine-tuning}

To further inspect the generalization ability of our method, we test the network on the images captured by the real cameras in our dataset. The center-view color image and the output disparity map between the center view and the right view are shown in Fig.~\ref{fig:res-real}. From the qualitative results, we can see the network still performs stably and obtains better disparity maps than the supervised method PSMNet after being trained on our synthetic dataset. This indicates that after the training, our self-supervised model can perform more stably in practical applications.
Another advantage of the self-supervised method is that online fine-tuning becomes feasible. Therefore, we fine-tune the network using the newly captured images when being employed in the real world. The results show the estimated disparity maps are further improved, which are presented in supplementary materials. This demonstrates the practical usefulness of our self-supervised multiscopic framework.

\begin{figure}[t]
\centering
\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={8cm 0cm 10cm 17cm}, clip]{figure/results/example3_view1}
%   \caption*{Center view}
\end{subfigure}
%
\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={8cm 0cm 10cm 17cm}, clip]{figure/results/example3_disp1_mark}
%   \caption*{Ground truth}
\end{subfigure}
%
\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={8cm 0cm 10cm 17cm}, clip]{figure/results/example3_disp_stereo_mark}
  \caption*{Stereo}
\end{subfigure}
%
\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={8cm 0cm 10cm 17cm}, clip]{figure/results/example3_outputR_mark}
  \caption*{Multiscopic}
\end{subfigure}
% \vspace{-0.2cm}
\caption{Comparison between stereo mode and our multiscopic mode. The first row displays the center view image ground-truth disparity. The second row displays the disparity map obtained by self-supervised learning using 2 images and that using 3 images. Occluded areas are much better with our multiscopic approach.}
\label{fig:res-ablation}
\vspace{-0.2cm}
\end{figure}

\setlength{\tabcolsep}{4pt}
\begin{table}[t]
\centering
\begin{tabular}{c c c c c c}
\toprule
{Image} & $\mathcal{L}_P$ & $\mathcal{L}_M$  & D1-all & D1-occ   \\
\midrule
$2$ & w/o cross & \xmark & $7.43\%$ & $91.66\%$ \\
$3$ & w/o cross & \xmark & $7.40\%$ & $91.54\%$ \\
$3$ & Cross & \xmark & $5.05\%$ & $38.71\%$ \\
$3$ & Cross & w/o uncertainty & $4.32\%$ & $15.29\%$ \\
$3$ & Cross & uncertainty-aware & $3.82\%$ & $10.87\%$ \\
\bottomrule
\end{tabular}
\caption{Ablation study on KITTI 2015. ``w/o cross" means only using $\mathcal{L}_P(I_{cl}^l, I_c)$, $\mathcal{L}_P(I_{cr}^r, I_c)$. ``w/o uncertainty" means only using the first equation of Equ.~\ref{equ:lossm} for $\mathcal{L}_M$. D1-occ is the D1 error of occluded pixels.}
\label{tab:ablation}
\vspace{-0.3cm}
\end{table}
\setlength{\tabcolsep}{4pt}


\subsection{Ablation Study}

To inspect the effect of our framework, we evaluate each module of our model on the KITTI 2015 training set, as displayed in Table~\ref{tab:ablation}. For the stereo self-supervised mode, we use only two images where the photometric loss is built by warping between the center image and the right image. Then we add modules proposed in our framework one by one.
The result shows that a better disparity map can be obtained with our cross-photometric loss as well as the uncertainty-aware mutual-supervision loss, especially in occluded areas. A qualitative comparison is shown in Fig.~\ref{fig:res-ablation}, from where we can see the occluded parts in stereo mode cannot be reconstructed correctly but are estimated much better in multiscopic mode. This is as expected. The loss $\mathcal{L}_P$ and $\mathcal{L}_M$ in multiscopic mode can both assist the estimation in occluded areas since they link the left and the right view, e.g., the invisible pixel in the left view would cause a large loss in $\mathcal{L}_M$ and $\mathcal{L}_P(I_{cr}^{l},I_c)$.




==> includes/intro.tex <==
% !TEX root =  ../main.tex

\section{Introduction}


% background and application
%Depth estimation is essential for numerous applications such as robotic manipulation, autonomous driving and 3D reconstruction. Depth sensors like structure-light cameras and time-of-flight sensors are equipped to perceive the surrounding environments, but they are expensive compared to RGB cameras. While the accuracy of monocular RGB camera is not high enough, most industrial solutions employ stereo cameras, which are two horizontally aligned cameras. With this structure, many constraints can be enforced to compute an accurate depth, e.g. the horizontal disparity of a pixel is determined by the depth such that the depth estimation could be solved by pixel correspondence matching. Therefore, could we obtain better depth estimation by introducing more RGB cameras at aligned positions since the RGB cameras are low-cost?
Accurate depth estimation is essential for numerous applications such as robotic manipulation, autonomous driving, 3D reconstruction. Various industrial solutions have employed stereo cameras for dense depth sensing. A vital benefit of a stereo camera is that the two cameras are axis-aligned so that the corresponding pixels between two images can lie on the same row. It appears that adding more axis-aligned cameras can help obtain high-quality depth maps. In this work, we study a novel problem for self-supervised stereo matching: given axis-aligned multiscopic images, can we train a stereo matching model for better depth sensing?


% motivation
Recent deep-learning-based methods for depth estimation have dominated most benchmarks~\cite{kendall2017end,chang2018pyramid,zhang2019ga}. However, these learning-based methods do not perform stably on unseen scenarios since the methods rely heavily on the training data. The ground-truth depth is hard to collect in the real world so that the size of the training data with ground-truth depth is usually small~\cite{geiger2012we}. In this case, the network trained with limited data is prone to overfitting the training data rather than understanding the underlying structure of the task. Thus, most deep-learning-based approaches do not have stable generalization ability, which restricts their applications in the industry.


To this end, researchers are exploring unsupervised learning for depth estimation~\cite{godard2017unsupervised,wang2019unos}. Compared to supervised approaches, unsupervised learning does not need the ground-truth depth, so it can be trained with a large amount of data. Also, since there is no ground-truth depth, the network needs to find the underlying pattern and geometry structure of images for stereo matching rather than simply overfitting the real depth value. Another advantage of unsupervised learning is that online fine-tuning becomes plausible~\cite{tonioni2019learning,tonioni2019real,zhong2017self}. As the ground truth is not needed for training a model, the model can be updated when processing the new inputs, which can lead to various practical applications.

The idea of exploiting more input data to assist the learning has been recently explored by some researchers~\cite{godard2017unsupervised,wang2019unos,liu2020flow2stereo}. For example, a model for unsupervised monocular depth estimation can be trained with stereo images~\cite{godard2017unsupervised}. Inspired by this idea, we wonder if the unsupervised stereo matching can be improved with three or more images during training.

% what this paper is about
% what makes this work relevant

\begin{figure}[]
\centering
  \includegraphics[width=0.7\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/camera.pdf}
\caption{Our multiscopic vision structure. Images are taken at parallel, co-planar, and same-parallax camera positions, such that the pixel disparities between adjacent images are the same.}
\label{fig:camera}
\vspace{-0.5cm}
\end{figure}

\begin{figure*}[t]
\centering
  \includegraphics[width=1.8\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/framework}
\caption{Self-supervised learning framework for the three-image multiscopic structure. Two networks sharing the same parameters compute the disparity $D_c^l,D_c^r$ and uncertainty map $\sigma^l,\sigma^r$ end-to-end, which are then used to warp the left and right images $I_l,I_r$ back to the center view, generating four reconstructed images $I_{cl}^l, I_{cl}^r, I_{cr}^l, I_{cr}^r$. The cross photometric loss $\mathcal{L}_P$ is built between them and the real center image $I_c$, the uncertainty-aware mutual-supervision loss $\mathcal{L}_M$ is built between $D_c^l$ and $D_c^r$ conditioned on $\sigma^l,\sigma^r$, and the smoothness loss $\mathcal{L}_S$ is built for each disparity map.}
\label{fig:framework}
\vspace{-0.5cm}
\end{figure*}

In this paper, we explore self-supervised learning depth estimation utilizing multiple images taken at aligned camera positions as input during training. We assume that multiple images are captured at horizontally or vertically aligned positions. As the stereo structure brings some benefits to depth estimation, the multiscopic structure introduces more constraints that can supervise the learning. These cameras are parallel, co-planar, and with the same baselines, as shown in Fig.~\ref{fig:camera}, such that the pixel disparities between adjacent images are the same. In this case, the disparity maps from the center view to any surrounding view should be exactly the same. Furthermore, for the left and right views, the pixel shift exists only in the horizontal axis, and for the bottom and top view, the pixel shift exists only in the vertical axis.

By exploiting these constraints, we can train a network to predict a better disparity map end-to-end without ground-truth depth information, as shown in Fig.~\ref{fig:framework}. Uncertainty-aware mutual supervision between different disparity maps serves as the self-supervising signal to optimize the network. Since the learning is self-supervised, it needs to find the underlying relationship of the multiscopic images to compute the disparity. Our experiment shows that the learned network can be generalized to unseen scenarios well, as there is no chance to overfit the ground-truth depth. After being trained with only synthetic images, our model performs well in real-world scenarios.

To make our unsupervised learning framework work and to promote more works in multiscopic vision, we propose a new dataset with 1300 scenes of multiscopic images as there is no available large dataset for multiscopic vision. There are a large number of synthetic images rendered by 3D engines~\cite{McCormac:etal:ICCV2017,Matterport3D} and a small number of real images taken by our multiscopic cameras. For the synthetic images, ground-truth depths are also provided.



Our main contributions concerning the self-supervised learning depth estimation framework and the multiscopic dataset are summarized as follows:

1) We exploit multiple images in a multiscopic structure for training a network to predict the disparity maps without the need for ground-truth depth. Optimization is built from the mutual supervision between confident areas of disparities obtained from different center-surround image pairs.

2) We build a new dataset of multiscopic images of 1200 scenes rendered in 3D engines and 100 scenes captured in the real world with our multiscopic cameras. Trained on only synthetic images, our model can be generalized to perform well on real-world data.

3) The experiment shows that our model outperforms other unsupervised approaches for stereo matching by a large margin and is comparable to supervised methods when generalized to unseen data.

% \begin{enumerate}
% \item
% We exploit multiple images in a multiscopic structure for training a network to predict the disparity maps without the need for ground-truth depth. Optimization is built from the mutual supervision between disparities obtained by different center-surround image pairs in confident areas.
% \item
% We build a new dataset of multiscopic images of 1200 scenes rendered in 3D engines and 100 scenes captured in real-world with our multiscopic cameras. Trained on only synthetic images, our model can be generalized to perform well on the real-world data.
% \item The experiment shows that our model outperforms other unsupervised approaches for stereo matching and is comparable to supervised methods when generalized to unseen data.

% \end{enumerate}





==> includes/related_work.tex <==
% !TEX root =  ../main.tex

\begin{figure*}[t]
\centering
\begin{subfigure}{0.65\columnwidth}
  \centering
  \includegraphics[height=4.5cm, trim={0cm 0cm 0cm 0cm}, clip]{figure/dataset/example41.jpg}
  \caption{Color images}
\end{subfigure}
%
% \begin{subfigure}{0.75\columnwidth}
%   \centering
%   \includegraphics[height=5cm, trim={0cm 0cm 0cm 0cm}, clip]{figure/dataset/test60.jpg}
% \end{subfigure}
% %
% \begin{subfigure}{0.35\columnwidth}
%   \centering
%   \includegraphics[height=5cm, trim={0cm 0cm 0cm 0cm}, clip]{figure/dataset/multieye1}
% \end{subfigure}
% %
\begin{subfigure}{0.65\columnwidth}
  \centering
  \includegraphics[height=4.5cm, trim={0cm 0cm 0cm 0cm}, clip]{figure/dataset/example41_depth}
  \caption{Ground-truth disparity maps}
\end{subfigure}
%
% \begin{subfigure}{0.75\columnwidth}
%   \centering
%   \includegraphics[height=5cm, trim={0cm 0cm 0cm 0cm}, clip]{figure/dataset/test60_depth}
%   \caption{}
% \end{subfigure}
% %
\begin{subfigure}{0.3\columnwidth}
  \centering
  \includegraphics[height=4.5cm, trim={0cm 0cm 0cm 0cm}, clip]{figure/dataset/slider_30_v}
  \caption{Real images}
\end{subfigure}
%
\caption{Example scenes of multiscopic images in our dataset.
% (a) is rendered by Habitat-sim, and (b) is rendered by SceneNet RGB-D.
The synthetic color images (a) and corresponding perfect disparity maps (b) displayed in Jet colormap are presented. (c) is one set of images obtained by the multiscopic system in real world.}
\label{fig:dataset}
\vspace{-0.5cm}
\end{figure*}


\begin{figure}[t]
\centering
\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[height=2cm, trim={0cm 0cm 0cm 0cm}, clip]{figure/multieye}
  \caption{Multi-eye}
\end{subfigure}
%
\begin{subfigure}{0.5\columnwidth}
  \centering
  \includegraphics[height=2cm, trim={0cm 0cm 0cm 0cm}, clip]{figure/movingeye}
  \caption{Moving-eye}
\end{subfigure}

\caption{Multiscopic systems designed to capture real multiscopic images. Multi-eye design (a) is using multiple identical cameras, while moving-eye design (b) is using one camera sliding on a precision linear rail.}
\label{fig:realcam}
\vspace{-0.5cm}
\end{figure}


\section{Related Work}

In this section, we first review some multiscopic depth estimation works and supervised learning-based stereo matching methods. Afterward, unsupervised learning approaches for depth estimation are discussed.

% \vspace{-0.2cm}
\textbf{Multiscopic depth estimation.} All previous depth estimation works using multiscopic images are based on traditional matching methods \cite{kolmogorov2002multi,maitre2008symmetric,wei2005asymmetrical,drouin2005geo,lee2014multi,fehrman2014depth}, since there is no available large dataset to train a network. Various methods take advantage of some constraints in multiscopic structure to improve the estimation results and only evaluate it on a small synthetic dataset, the Tsukuba images \cite{nakamura1996occlusion}.

% \vspace{-0.2cm}
\textbf{Deep stereo matching.} Deep learning-based methods explore using neural networks to replace one \cite{zbontar2016stereo} or all steps \cite{kendall2017end,chang2018pyramid,zhang2019ga} in traditional stereo matching to compute the disparity map. Exploiting the network to compute the matching cost of two image patches was first proposed in MC-CNN \cite{zbontar2016stereo}. Instead of handcrafted features, it extracts the learned deep features for calculating the similarity, after which the traditional steps are employed to get the final disparity output. To further take advantage of the neural networks, end-to-end approaches are proposed to remove all traditional matching steps \cite{kendall2017end,chang2018pyramid,zhang2019ga}. GC-Net \cite{kendall2017end} builds the 4D cost volume and then processes the cost volume using multi-scale 3D convolutions, in which way the geometry and context information is incorporated to calculate the disparity map. This is enhanced in PSMNet \cite{chang2018pyramid} by introducing spatial pyramid pooling and stacked hourglass 3D convolution. Additionally, optimization methods in traditional stereo matching, such as semi-global matching, are also introduced to assist the deep methods in more meaningful ways \cite{zhang2019ga}. Heretofore, end-to-end learning approaches have dominated most benchmarks and show significant advantages.



\textbf{Unsupervised depth estimation.} Despite the success of learning-based approaches in some specific datasets, they need plenty of ground-truth training data, which is expensive to acquire. To overcome this, more researchers are seeking assistance from unsupervised learning. Some unsupervised frameworks were first proposed for monocular depth estimation. The monocular depth network is supervised by the reconstruction loss between the stereo image pairs \cite{garg2016unsupervised,xie2016deep3d,guo2018learning}. The reconstructed images are synthesized by warping one view to the other view using the disparity maps. This is enhanced by introducing the consistency of disparity maps between the left view and the right view \cite{godard2017unsupervised}.

Instead of relying on the stereo images, some works combine the ego-motion and optical flow estimation to help the unsupervised depth learning from videos \cite{zhou2017unsupervised,yin2018geonet}. The loss is built by warping adjacent views with the computed depth, pose, and optical flow. Also, some geometric consistency losses are introduced to improve the estimation \cite{yin2018geonet}.

For stereo depth estimation, there are some losses similar to monocular approaches, and more constraints that can further supervise the learning. Zhou et al.~\cite{zhou2017unsupervised} evaluate the matching result and pick the confident patch pairs as the new training data, in which way the network is iteratively optimized. Godard et al.~\cite{godard2017unsupervised} realize the stereo matching using the same reconstruction loss and left-right consistency loss as the monocular depth task. This is further improved by introducing occlusion-aware loss \cite{luo2018unsupervised} or heuristic loss \cite{zhong2017self}. Then more works try to explore supervision from the consistency in stereo videos \cite{zhong2018open, wang2019unos, liu2020flow2stereo, kim2020loop}, by utilizing the consistency in stereo depth, optical flow, and ego-motion. Some other works also introduce parallax-attention \cite{wang2020parallax} or seek the assistance from other networks \cite{aleotti2020reversing}.

However, no prior work has explored the unsupervised deep depth estimation in multiscopic structure, in which there are even more constraints that can assist the unsupervised learning. Similar to supervising the monocular depth estimation with stereo images, we show that we can supervise the stereo matching with multiscopic images to obtain a better disparity map by exploiting the inner shape of the multiscopic structure. To the best of our knowledge, our work is the first unsupervised deep stereo depth estimation mehod utilizing multiscopic images.


==> includes/unsuperlearn.tex <==
% !TEX root =  ../main.tex



\section{Self-supervised Multiscopic Matching}

%In this section, we propose our unsupervised disparity estimation method using multiscopic images. In this paper, we only deal with three-image multiscopic system although our approach can be seamlessly employed on five or even more images.


\subsection{Learning Framework}
In rectified stereo matching, pixels shift along the horizontal axis such that the searching for pixels correspondence is simplified. The depth map can be constructed from a computed disparity map that establishes pixel correspondences between the left image $I_l$ and the right image $I_r$. With a disparity map, the right image can be warped back to the left image to produce a synthetic left image $I_l'$.
% \begin{equation}
% I_l'(u,v) = I_r(u-D_l(u,v), v).
% \end{equation}
%
Ideally, if the disparity map $D_l$ is correctly estimated, the synthetic left image $I_l'$ should be the same as $I_l$ except for occluded regions. Then the discrepancy between them can be used as a photometric loss in training a self-supervised model \cite{godard2017unsupervised}.

In multiscopic vision, a similar photometric loss can be enforced between any two axis-aligned images. Since the baselines between adjacent camera positions are the same, more constraints could be established in a constrained way. As shown in Fig.~\ref{fig:framework}, we deal with a multiscopic system with three images without loss of generality. Benefiting from the multiscopic architecture, the disparities between the center image and any surrounding image should be the same, with the center image as the reference. Therefore, one disparity map can be used to warp all surrounding images back to the center image to work as a cross photometric loss. The disparity $D_c^r$ between the center image $I_c$ and the right image $I_r$ can be used to not only warp $I_r$ to produce a synthetic center image $I_{cr}^{r}$, but also warp $I_l$ to produce $I_{cl}^{r}$, as shown in Fig.~\ref{fig:warp}. On the one hand, this cross warping consistency can strengthen the photometric supervision. On the other hand, it can address the occlusion problem which troubles stereo vision, e.g., the invisible pixel in the right view would cause a large loss between $I_{cl}^{r}$ and $I_c$.

In a multiscopic structure, another constraint is that the disparity maps between the center image and all surrounding images should be the same. The discrepancy in disparity values indicates inaccurate disparity estimation. Thus the difference between multiple disparities could work as mutual supervision, as shown in Fig.~\ref{fig:framework}. This also helps handle the occlusion problem, which is usually problematic in stereo matching. The occluded regions of the center image in one surrounding image can be seen in other images. For example, the occluded areas between the left image and the center image are hard to be estimated correctly in $D_c^l$, but these parts are estimated well in $D_c^r$. In this case, we estimate an uncertainty map for each disparity map. In the uncertain areas like occluded pixels in $D_c^l$, we take the confident pixels in $D_c^r$ as supervision labels and optimize the estimation network for $D_c^l$.

\begin{figure}[t]
\centering
\begin{subfigure}{1\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/loss1}
\end{subfigure}
\caption{Cross warping between $I_l,I_c,I_r$ using disparity maps $D_c^l, D_c^r$. The cross photometric loss is then established between the warping results $I_{cl}^{l},I_{cl}^{r},I_{cr}^{r},I_{cr}^{l}$ and the center image $I_c$.}
\label{fig:warp}
\vspace{-0.5cm}
\end{figure}

\begin{figure*}[t]
\centering
\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 1cm}, clip]{figure/result/exam0_view1}
\end{subfigure}
%
\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 1cm}, clip]{figure/result/exam0_disp1_mark}
\end{subfigure}
%
\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 1cm}, clip]{figure/result/exam0_disp_mark}
\end{subfigure}
%
\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 1cm}, clip]{figure/result/exam0_disp_psmnet_mark}
\end{subfigure}

\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/result/test28_view1}
  \caption*{Center view}
\end{subfigure}
%
\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/result/test28_disp1_mark}
  \caption*{Ground truth}
\end{subfigure}
%
\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/result/test28_disp_mark}
  \caption*{Our model}
\end{subfigure}
%
\begin{subfigure}{0.4\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/result/test28_disp_psmnet_mark}
  \caption*{PSMNet}
\end{subfigure}
\caption{Example outputs on synthetic test images. The center-view color images, the ground-truth disparity maps, the output disparity maps of our self-supervised model, and the output of the supervised method PSMNet are shown.}
\label{fig:res-synthe}
\vspace{-0.2cm}
\end{figure*}


\setlength{\tabcolsep}{3pt}
\begin{table*}[]
\small
\centering
\begin{tabular}{c c c c c c c c c}
\toprule
Method & Training set & {Gound truth} & EPE  & Bad$0.5$ & Bad$1$ & Bad$2$  \\
\midrule
Godard et al.~\cite{godard2017unsupervised} & Synthetic & \xmark &
$2.16$ & $35.22\%$ & $21.67\%$ & $10.83\%$ \\
% Ours & Synthetic & \xmark & $1.29$ & $\mathbf{15.64\%}$ & $\mathbf{9.32\%}$ & $\mathbf{6.37\%}$  \\
Ours & Synthetic & \xmark & $1.19$ & $\mathbf{16.54\%}$ & $\mathbf{9.46\%}$ & $\mathbf{6.07\%}$  \\
% bad3: 4.84\%
\midrule
PSMNet \cite{chang2018pyramid} & Synthetic & \cmark & $\mathbf{1.07}$  & $23.01\%$ & $11.69\%$ & ${6.36\%}$ \\
\midrule
MC-CNN \cite{zbontar2016stereo} & KITTI & \cmark & $3.55$ & $42.88\%$ & $27.18\%$ & $20.05\%$ \\
PSMNet \cite{chang2018pyramid} & Cityscapes + KITTI & \cmark & $2.94$ & $75.53\%$ & $50.12\%$ & $18.09\%$ \\
\bottomrule
\end{tabular}
\caption{Results on the synthetic test set.}
\label{tab:synthetic}
\vspace{-0.5cm}
\end{table*}
\setlength{\tabcolsep}{3pt}


\subsection{Network Structure}
While the design of the network structure is not our focus in this work, we use PSMNet \cite{chang2018pyramid} as our network backbone, which is an end-to-end disparity regression model. We trim the structure by reducing some layers for efficiency and add an uncertainty head. Details of the network are provided in the supplementary materials. The spatial pyramid pooling module and 3D CNN module incorporate both the local and global information to produce a cost volume, which is then converted to a probability volume to regress the final disparity prediction. The uncertainty head regresses an uncertainty map from the cost volume.

In our three-image multiscopic system, there are two matchings. One is between the center image and the left image, and the other is between the center image and the right image. We use two matching networks sharing the same parameters to calculate the disparity maps $D_c^l$ and $D_c^r$.





\subsection{Loss Function}

In our multiscopic self-supervised framework, we utilize the cross photometric loss $\mathcal{L}_P$ and the uncertainty-aware mutual-supervision loss $\mathcal{L}_\sigma, \mathcal{L}_M$ to guide the learning process. Additionally, a regularization term $\mathcal{L}_S$ is also introduced to improve the smoothness of the output disparity. Our overall loss is the sum of these terms with weighting factors $\lambda_1, \lambda_2, \lambda_3, \lambda_4$:
\begin{equation}
    \mathcal{L} = \lambda_1\mathcal{L}_P + \lambda_2\mathcal{L}_\sigma + \lambda_3\mathcal{L}_M + \lambda_4\mathcal{L}_S.
\end{equation}

\subsubsection{Cross Photometric Loss}
$\mathcal{L}_P$ is used to evaluate how similar the reconstructed images $I_{cl}^{l},I_{cl}^{r},I_{cr}^{r},I_{cr}^{l}$ are to the real center image $I_c$, where
\begin{equation}
\begin{aligned}
    I_{cl}^{l}(u,v) &= I_l(u+D_c^l(u,v), v),\\
    I_{cl}^{r}(u,v) &= I_l(u+D_c^r(u,v), v).
    % I_{cr}^{l}(u,v) &= I_r(u-D_c^l(u,v), v),
    % I_{cr}^{r}(u,v) &= I_r(u-D_c^r(u,v), v).
\end{aligned}
\end{equation}
$I_{cr}^{r},I_{cr}^{l}$ are calculated in a similar way. The warping process is illustrated in Fig.~\ref{fig:warp}.

We use structural similarity (SSIM) \cite{wang2004image} loss to calculate the image discrepancy as
\begin{equation}
    \mathcal{L}_P(I_{cl}^l, I_c) = \frac{1-SSIM(I_{cl}^l, I_c)}{2},
    % + (1-\alpha)\Big|I_{cl}^l-I_c\Big|,
\end{equation}
where the SSIM window size is set to $5$.
The other three parts are calculated in a similar way, and the final cross photometric loss is computed by taking the average:
\begin{equation}
    \mathcal{L}_P=\frac{\mathcal{L}_P(I_{cl}^l)+
                        \mathcal{L}_P(I_{cl}^r)+
                        \mathcal{L}_P(I_{cr}^l)+
                        \mathcal{L}_P(I_{cr}^r)}{4}.
\end{equation}





\begin{figure*}[t]
\centering
\begin{subfigure}{0.6\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/test000006_10}
\end{subfigure}
%
\begin{subfigure}{0.6\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/test000006_10_1}
\end{subfigure}
%
\begin{subfigure}{0.6\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/test000006_10_2}
\end{subfigure}

\begin{subfigure}{0.6\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/test000012_10}
  \caption*{Left image}
\end{subfigure}
%
\begin{subfigure}{0.6\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/test000012_10_1}
  \caption*{Disparity map}
\end{subfigure}
%
\begin{subfigure}{0.6\columnwidth}
  \centering
  \includegraphics[width=1\columnwidth, trim={0cm 0cm 0cm 0cm}, clip]{figure/results/test000012_10_2}
  \caption*{Error map}
\end{subfigure}
% \vspace{-0.2cm}
\caption{Qualitative results on KITTI 2015 test set.}
\label{fig:res-kitti}
\vspace{-0.3cm}
\end{figure*}





\subsubsection{Uncertainty-aware Mutual-supervision Loss}
$\mathcal{L}_M$ utilizes the output of one network to supervise the other network. The discrepancy between the disparity output $D_c^l$ generated by the center-left network and $D_c^r$ generated by the center-right network means erroneous matching. Thus we learn an uncertainty map for each disparity output. In uncertain areas, we supervise the uncertain output with the other output, and in confident areas, we calculate the consistency loss between two outputs.

Following the heteroscedastic aleatoric uncertainty setup in \cite{kendall2017uncertainties}, we model the reconstruction task with uncertain L1 loss as
\begin{equation}
\begin{aligned}
    \mathcal{L}_\sigma(I_{cl}^l) = \sum_{u,v} \frac{\sqrt{2}}{\sigma^l(u,v)}|I_{cl}^l(u,v)-I_c(u,v)| + \log \sigma^l(u,v) ,
\end{aligned}
\end{equation}
where $\sigma^l$ is the estimated uncertainty map generated by center-left image pair. Then $\mathcal{L}_\sigma$ is computed by taking the average of $\mathcal{L}_\sigma(I_{cl}^l), \mathcal{L}_\sigma(I_{cl}^r), \mathcal{L}_\sigma(I_{cr}^l), \mathcal{L}_\sigma(I_{cr}^r)$.

With the uncertainty map $\sigma_l, \sigma_r$, we can do the mutual-supervising as

\begin{equation}
\begin{aligned}
\mathcal{L}_M=
  \begin{cases}
  ||D_c^l-D_c^r|| , \quad & \text{if} \ \sigma_l, \sigma_r < T_\sigma \\
  ||D_c^l-\text{label}(D_c^r)|| , \quad & \text{if} \ \sigma_l \geq T_\sigma, \sigma_r < T_\sigma \\
  ||D_c^r-\text{label}(D_c^l)|| , \quad & \text{if} \ \sigma_r \geq T_\sigma, \sigma_l < T_\sigma .
  \end{cases}
\end{aligned}
\label{equ:lossm}
\end{equation}
where $T_\sigma=e$ is a threshold over which the disparity estimation is regarded as uncertain, and the label operation converts the confident estimation to supervision signal that is used to optimize the estimation of the other network. In regions where both estimations are uncertain, we do not calculate the loss. This loss could be especially useful in occluded regions. When the matching between the center-left images is wrong due to occlusion, it can be corrected by the label from the center-right matching.
% Thus, this loss is formulated as
% \begin{equation}
%     \mathcal{L}_S = \min\{\Big|D_c^l-D_c^r\Big|,\ d_{T}\},
% \end{equation}
% where $d_T$ is a truncation threshold set to $10$.


% If the weight of this loss is too large at the beginning of the training, it would dominate the learning and lead to overly flat $D_c^l, D_c^r$, which has the minimum difference. So we begin with a small weighting factor and increase it after the network can obtain meaningful results.






\subsubsection{Smoothness Loss}
$\mathcal{L}_S$ encourages the adjacent pixels to have similar disparities, especially for those with a similar color. The punishment is enforced for discontinuous disparities and determined by the disparity variation and color difference, as
\begin{equation}
\begin{split}
    \mathcal{L}_S=\
    &f_x(D_c^l)e^{-\gamma||\partial_x I_c||}+f_y(D_c^l)e^{-\gamma||\partial_y I_c||}+\\
    &f_x(D_c^r)e^{-\gamma||\partial_x I_c||}+f_y(D_c^r)e^{-\gamma||\partial_y I_c||},
\end{split}
\end{equation}
where $\gamma$ is a scale factor related to the image intensity normalization and is set to $10$ in our work. $f_{x/y}$ is composed of a discontinuous loss $K$ plus the disparity differential as
\begin{equation}
f_x(D)=
\begin{cases}
    K+||\partial_x D|| , \quad & \text{if} \ ||\partial_x D||>0.5\\
    ||\partial_x D||  , \quad & \text{otherwise}.
\end{cases}
\end{equation}
The disparity difference larger than $0.5$ is considered discontinuity and is punished by an additional $K=10$.

